On the complexity of unique quantum witnesses and quantum approximate counting

We study the long-standing open question on the power of unique witnesses in quantum protocols, which asks if $\textsf{UniqueQMA}$, a variant of $\textsf{QMA}$ whose accepting witness space is 1-dimensional, contains $\mathsf{QMA}$ under quantum reductions. This work rules out any black-box reduction from $\mathsf{QMA}$ to $\mathsf{UniqueQMA}$ by showing a quantum oracle separation between $\mathsf{BQP}^\mathsf{UniqueQMA}$ and $\mathsf{QMA}$. This provides a contrast to the classical case, where the Valiant-Vazirani theorem shows a black-box randomized reduction from $\mathsf{UniqueNP}$ to $\mathsf{NP}$, and suggests the need for studying the structure of the ground space of local Hamiltonians in distilling a potential unique witness. Via similar techniques, we show, relative to a quantum oracle, that $\mathsf{QMA}^\mathsf{QMA}$ cannot decide quantum approximate counting, ruling out a quantum analogue of Stockmeyer's algorithm in the black-box setting. We then ask a natural question; what structural properties of the local Hamiltonian problem can we exploit? We introduce a physically motivated candidate by showing that the ground energy of local Hamiltonians that satisfy a computational variant of the eigenstate thermalization hypothesis (ETH) can be estimated through a $\mathsf{UniqueQMA}$ protocol. Our protocol can be viewed as a quantum expander test in a low energy subspace of the Hamiltonian and verifies a unique entangled state across two copies of the subspace. This allows us to conclude that if $\mathsf{UniqueQMA}$ is not equivalent to $\mathsf{QMA}$, then $\mathsf{QMA}$-hard Hamiltonians must violate ETH under adversarial perturbations. This also serves as evidence that chaotic local Hamiltonians, such as the SYK model may be computationally simpler than general local Hamiltonians.

==> counting.tex <==
\subsection{Background}
\begin{itemize}
    \item Discuss Stockmeyer.
    \item Definitions of quantum approximate counting: $\SharpBQP$, Bravyi et al. 21, Brown-Flammia-Schuch 11 , Shi-Zhang 09.
    \item Remark different Aaronson et al.
\end{itemize}




\subsection{Definition of $\BQP^{\QMA}$}
Discuss oracle definitions: (+discuss subtleties in defining quantum PH, promiseQMA vs QMA oracles, etc.) Make our choice $\rightarrow$ Convert into circuit definition below.

We have the following registers:
\begin{itemize}
    \item $\reg R_\mathrm{ctrl}$: control register, wlog for both $\QMA$ oracles and subspace oracle (but maybe should separate...)
    \item $\reg R_\mathrm{w}$: witness register for $\QMA$ oracles
    \item $\reg R_\mathrm{comp}$: the rest.
\end{itemize}

Let $Q$ be number of $\QMA^{\mc O}$ calls, let $L$ be number of subspace oracle $\mc O$ queries outside of $\QMA^{\mc O}$, let $q_i$ be number of subspace oracle queries within the $i$-th $\QMA^{\mc O}$-oracle call. Wlog we can take $L=Q$.
We use the following notations to denote the circuit primitives with in the $\BQP^{\QMA^{\mc O}}$ machine:
\begin{itemize}
    \item $\{U_i\}_{ 0\leq i\leq L+Q}$ denote unitary layers in between calls to $\mc O$ and to $\QMA^{\mc O}$. Act on all registers.
    \item $\{W^{\mc O}_i\}_{1\leq i \leq Q}$ denote the (potentially non-physical, but controlled on $\reg R_\mathrm{ctrl}$) operations preparing the witness on $\reg R_\mathrm{w}$ (potentially in superposition) for the $i$-th $\QMA^{\mc O}$ call. We will only care about its behavior when the witness register is initialized to the all-0s state.
    \item $\{V_{i,j}\}_{1\leq i \leq Q, 0\leq j \leq q_j}$ denote classically controlled (on $\reg R_\mathrm{ctrl}$) unitary layers in between calls to $\mc O$ inside the $i$-th $\QMA^{\mc O}$ call. (Note $V_{i,j}$ are independent of $\mc O$).
\end{itemize}

Include fig.

Under the above notation, the $\BQP^{\QMA^{\mc O}}$ is
\begin{align}
        \mc V &\dfn (\Id \otimes \ketbra 1_{\reg R_\tout})  \dots \big( U_{2i}  \O^{\Pi}  U_{2i-1} \left(  V_{i,q_i} \mc O^{\Pi}\hdots  
 V_{i,1} \mc O^{\Pi} V_{i,0} \right) W^{\mc O}_{i} \big)  \hdots U_0 (\ketbra{0^{n}}).
    \end{align}

We can insert the projector $\ketbra{0}_{\reg R_\mathrm{w}}$ before each $W_i^{\mc O}$.



\subsection{Query lowerbound}
\begin{definition}
    Subspace dimension distinguishing problem.
\end{definition}


\paragraph{Warm-up: $\QMA$ query lowerbound.} Can drop if we dont have time, writing this up would take a page or so...


Let $W_i^{\mc O_S}$ be the witness preparation operations in the YES case (oracle $\mc O_S$ has dimension small, (1 is ok?))

Let $W_i^{\mc O_T}$ be the witness preparation operations in the NO case (oracle $\mc O_T$ has dimension large)


\paragraph{Outer hybridization.}
We first define the outer hybridized machine
\begin{align*}
   \mc V_t^{S,T} \triangleq \dots \big( U_{2t+2}  \O_T^{\Pi}  U_{2t+1} &\left(  V_{t+1,q_{t+1}} \mc O_T^{\Pi}\hdots  
 V_{t+1,1} \mc O_T^{\Pi} V_{t+1,0} \right) W^{\mc O_T}_{t+1} \big)\\
 &\big( U_{2t}  \O_S^{\Pi}  U_{2t-1} \left( V_{t,q_t} \mc O_S^{\Pi}  \hdots  
 V_{t,1} \mc O_S^{\Pi} V_{t,0} \right) W^{\mc O_S}_{t} \big)  \hdots .
\end{align*}
Again, we can insert the projector $\ketbra{0}_{\reg R_\mathrm{w}}$ before each $W_i^{\mc O_{S/T}}$.

The completeness condition reads that there exist $\{W^{\mc O_S}_i\}$ such that $\|\ketbra 1_{\reg R_\tout}  \mc V_{L}^{S,T} \ketbra{0^n} \|^2 \geq 1-\varepsilon$. And the soundness reads that for any $\{W^{\mc O_T}_i\}$ such that $\|\ketbra 1_{\reg R_\tout} \mc V_{0}^{S,T}\ketbra{0^n} \|^2 \leq \varepsilon$.


\begin{claim} Let $\ket{\psi_t} \triangleq  \mc V_t^{S,T} \ket{0^n}$. There exists $t^\star \leq L$ such that
\begin{align}
    \frac{1-O(\varepsilon)}{L} \leq \|\ket{\psi_{t^\star}} - \ket{\psi_{t^\star -1 } }\|.
\end{align}
Let $\ket{\phi_{t^\star -1}} = \big( U_{2t^\star-2}  \O_S^{\Pi}  U_{2t^\star-3} \left(  V_{t^\star-1,q_{t^\star-1}} \mc O_S^{\Pi} \hdots  
 V_{t^\star-1,1} \mc O_S^{\Pi} V_{t^\star-1,0} \right) W^{\mc O_S}_{t^\star-1} \big)  \hdots U_0 \ket{0^{n}} $. The above implies that
\begin{align}
    \|\left( \O_S^{\Pi}  U_{2t-1} \left( V_{t,q_t} \mc O_S^{\Pi} \hdots  
 V_{t,1} \mc O_S^{\Pi} V_{t,0} \right) W^{\mc O_S}_{t}  -  \O_T^{\Pi}  U_{2t-1} \left( V_{t,q_t} \mc O_T^{\Pi} \hdots  
 V_{t,1} \mc O_T^{\Pi} V_{t,0} \right) W^{\mc O_T}_{t}  \right)   \ket{\phi_{t^\star -1}}\| \geq \frac{1-O(\varepsilon)}{L}.
\end{align}
\end{claim}

\paragraph{Inner hybridization.} Similarly we define
\begin{align}
    \mc C_{q}^{S,T} \triangleq  \O_T^{\Pi}  U_{2t-1} \big(\hdots  V_{t,q+1} \mc O_T^{\Pi}  
 V_{t,q} \mc O_S^{\Pi} \hdots V_{t,0} \big) W^{\mc O_S}_{t} , \qquad 1\leq q \leq q_t
\end{align}
with $\mc C_{0}^{S,T} \triangleq \O_T^{\Pi}  U_{2t-1} \big(\hdots  V_{t,q+1} \mc O_T^{\Pi}  \hdots V_{t,0} \big) W^{\mc O_T}_{t} $ and $\mc C_{q_t+1}^{S,T} \triangleq \O_S^{\Pi}  U_{2t-1} \big(\hdots  V_{t,q+1} \mc O_S^{\Pi}  \hdots V_{t,0} \big) W^{\mc O_S}_{t}$, where $t=t^\star$ from above.

\begin{claim} Let $\ket{\varphi_q}\triangleq \mc C_{q}^{S,T} \ket{\phi_{t^\star -1}}$ (which is a state independent of $T$). There exists $1\leq q^\star \leq q_{t^\star} +1$ such that 
\begin{align}
    \frac{1-O(\varepsilon)}{L(q_{t^\star}+1)} \leq \|\ket{\varphi_q} - \ket{\varphi_{q-1}} \|.
\end{align}
    \begin{itemize}
        \item Case 1: $2\leq q^\star \leq q_{t^\star}$. We're done -- using same argument as in UQMA section.
        \item Case 2: $q^\star = q_{t^\star} +1$. Same.
        \item Case 3: $q^\star = 1 $...?
    \end{itemize}
\end{claim}

\subsection{Oracle separation}
\begin{itemize}
    \item Diagonalizing oracle
    \item Interpret oracle problem as $\SharpBQP^{\mc O}$ problem
\end{itemize} 


